Viraliency: Pooling Local Virality

In our overly-connected world, the automatic recognition of virality - the quality of an image or video to be rapidly and widely spread in social networks - is of crucial importance, and has recently awaken the interest of the computer vision community. Concurrently, recent progress in deep learning architectures showed that global pooling strategies allow the extraction of activation maps, which highlight the parts of the image most likely to contain instances of a certain class. We extend this concept by introducing a pooling layer that learns the size of the support area to be averaged: the learned top-N average (LENA) pooling. We hypothesize that the latent concepts (feature maps) describing virality may require such a rich pooling strategy. We assess the effectiveness of the LENA layer by appending it on top of a convolutional siamese architecture and evaluate its performance on the task of predicting and localizing virality. We report experiments on two publicly available datasets annotated for virality and show that our method outperforms state-of-the-art approaches.

==> huge_figure.tex <==
\begin{figure*}[t]
 \setlength{\mywidth}{0.9cm}
 \centering
 \begin{tabular}{cccccccccccccccc}
 Original Image & \multicolumn{5}{c}{GAP} & \multicolumn{5}{c}{GMP} & \multicolumn{5}{c}{G\textsc{lena}P}\\\hspace{-4mm}
%    \multirow{2}[2]{*}[5mm]{\includegraphics[width=3\mywidth,height=3\mywidth]{img/channels/serena}}&\hspace{-2mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/2top1channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/2top2channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/2top3channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/2top4channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/2top5channel.png}&\hspace{-2mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/2top1channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/2top2channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/2top3channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/2top4channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/2top5channel.png}&\hspace{-2mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/2top1channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/2top2channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/2top3channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/2top4channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/2top5channel.png}\vspace{-1mm}\\
%    &\hspace{-2mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/2top6channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/2top7channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/2top8channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/2top9channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/2top10channel.png}&\hspace{-2mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/2top6channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/2top7channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/2top8channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/2top9channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/2top10channel.png}&\hspace{-2mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/2top6channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/2top7channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/2top8channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/2top9channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/2top10channel.png}\vspace{-1mm}\\
%    &\hspace{-2mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/2top11channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/2top12channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/2top13channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/2top14channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/2top15channel.png}&\hspace{-2mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/2top11channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/2top12channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/2top13channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/2top14channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/2top15channel.png}&\hspace{-2mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/2top11channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/2top12channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/2top13channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/2top14channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/2top15channel.png}\\
%    \multirow{2}[2]{*}[5mm]{\includegraphics[width=3\mywidth,height=3\mywidth]{img/channels/bluewaves.jpg}}&\hspace{-2mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/18top1channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/18top2channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/18top3channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/18top4channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/18top5channel.png}&\hspace{-2mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/18top1channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/18top2channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/18top3channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/18top4channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/18top5channel.png}&\hspace{-2mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/18top1channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/18top2channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/18top3channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/18top4channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/18top5channel.png}\vspace{-1mm}\\
%    &\hspace{-2mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/18top6channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/18top7channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/18top8channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/18top9channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/18top10channel.png}&\hspace{-2mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/18top6channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/18top7channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/18top8channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/18top9channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/18top10channel.png}&\hspace{-2mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/18top6channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/18top7channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/18top8channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/18top9channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/18top10channel.png}\vspace{-1mm}\\
%    &\hspace{-2mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/18top11channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/18top12channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/18top13channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/18top14channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gap/18top15channel.png}&\hspace{-2mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/18top11channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/18top12channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/18top13channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/18top14channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/gmp/18top15channel.png}&\hspace{-2mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/18top11channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/18top12channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/18top13channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/18top14channel.png}&\hspace{-4mm}%
%    \includegraphics[width=\mywidth]{img/channels/init1/18top15channel.png}\\
   \multirow{2}[2]{*}[5mm]{\includegraphics[width=4\mywidth,height=3\mywidth]{img/channels/videogames.jpg}}&\hspace{-3mm}%
   \includegraphics[width=\mywidth]{img/channels/gap/25top1channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gap/25top2channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gap/25top3channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gap/25top4channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gap/25top5channel.png}&\hspace{-3mm}%
   \includegraphics[width=\mywidth]{img/channels/gmp/25top1channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gmp/25top2channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gmp/25top3channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gmp/25top4channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gmp/25top5channel.png}&\hspace{-3mm}%
   \includegraphics[width=\mywidth]{img/channels/init1/25top1channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/init1/25top2channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/init1/25top3channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/init1/25top4channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/init1/25top5channel.png}\vspace{-1mm}\\
   &\hspace{-3mm}%
   \includegraphics[width=\mywidth]{img/channels/gap/25top6channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gap/25top7channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gap/25top8channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gap/25top9channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gap/25top10channel.png}&\hspace{-3mm}%
   \includegraphics[width=\mywidth]{img/channels/gmp/25top6channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gmp/25top7channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gmp/25top8channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gmp/25top9channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gmp/25top10channel.png}&\hspace{-3mm}%
   \includegraphics[width=\mywidth]{img/channels/init1/25top6channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/init1/25top7channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/init1/25top8channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/init1/25top9channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/init1/25top10channel.png}\vspace{-1mm}\\
   &\hspace{-3mm}%
   \includegraphics[width=\mywidth]{img/channels/gap/25top11channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gap/25top12channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gap/25top13channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gap/25top14channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gap/25top15channel.png}&\hspace{-3mm}%
   \includegraphics[width=\mywidth]{img/channels/gmp/25top11channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gmp/25top12channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gmp/25top13channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gmp/25top14channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/gmp/25top15channel.png}&\hspace{-3mm}%
   \includegraphics[width=\mywidth]{img/channels/init1/25top11channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/init1/25top12channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/init1/25top13channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/init1/25top14channel.png}&\hspace{-4mm}%
   \includegraphics[width=\mywidth]{img/channels/init1/25top15channel.png}\\
 \end{tabular}
 \caption{Top 15 channels (highest weight) contributing to the viraliency maps for Alex7 for the three global pooling strategies: GAP (left), GMP 
(middle) and G\textsc{lena}P$-$1 (right). Pixel values are color-coded in 
decreasing value from red to blue through green. White indicates unsued pixels, \ie those that do not affect the average and to whom the error 
is not backpropagated.\label{fig:contributors}}\vspace{-3mm}
\end{figure*}

==> old.tex <==
\section{Previous shit}

\subsection{UIV dataset}
Be careful: These numbers are slightly different than the final ones because when computing these numbers I forgot to evaluate the last 39 images 
(both in the numerator and denominator of the accuracy).

\begin{table}
 \caption{Results using ConvAlexNet (5 conv layers). [a] Means simple siamese. [e] Finetunning also Conv2. [f] Finetunning from Conv4.}
 %[d] Means siamese with fixed reference network and objectness.}
 \begin{tabular}{cccc}
 \toprule
  Pooling & [a] & [e] & [f]\\%& [d] \\
 \midrule
  GAP & 54.4 & 50.5 & 54.5\\
  GMP & 50.4 & 50.4 & 51.1\\%& 72.0\\
 \midrule
  G\!\blena{0.6}\!P-$0$ & 52.4 & 51.2 & 48.4 \\%& 68.3\\
  GLENAP-$0.5$ & 50.9 & 50.1 & 49.1 \\%& 69.8 \\
  G\textsc{lena}P-$1$ & 50.1 & 51.1 & 52.8\\%& 70.6 \\
  GLP\\
 \bottomrule
 \end{tabular}
\end{table}

\begin{table}
 \caption{Results using MITAlexNet (7 conv layers). [a] Means simple siamese. [g] FineTunning from Conv5. [h] FineTunning from Conv6. [i] Strategy 
[a] with lower learning rate, except for LENA params.}
 %[d] Means siamese with fixed reference network and objectness.}
 \begin{tabular}{ccccc}
 \toprule
  Pooling & [a] & [g] & [h] & [i]\\%& [d] \\
 \midrule
  GAP & 71.8 & 66.6 & 65.1 & 61.5\\
  GMP & 79.2 & 80.3 & 78.4 & 62.3 \\%& 72.0\\
 \midrule
  LENA-$0$ & 67.7 & 68.0 & 68.2 & 62.8 \\%& 68.3\\
  LENA-$0.5$ & 67.9 & 66.2 & 65.6 & 61.6\\%& 69.8 \\
  LENA-$1$ & 68.4 & 68.3 & 67.9 & 62.6\\%& 70.6 \\
  \midrule
  LENA-GMP & 75.3 \\
 \bottomrule
 \end{tabular}
\end{table}

\begin{table}
 \caption{Results using VGGNet. [a] Means simple siamese. [b] Means siamese plus objectness. [c] Objectness (30 classes).}
 %[d] Means siamese with fixed reference network and objectness.}
 \begin{tabular}{cccc}
 \toprule
  Pooling & [a] & [b] & [c]\\
 \midrule
  GAP & 48.1 &  & \\
  GMP & 60.8 &  & \\
 \midrule
  LENA-$0$ & 58.9 &  &  \\
  LENA-$0.5$ & 73.1 &  & \\
  LENA-$1$ & 73.7 &  & \\
 \bottomrule
 \end{tabular}
\end{table}

\clearpage
\subsection{Googleplus dataset}
AND Devi's method in Jacopo's dataset is: 65.4\%

\begin{table}
 \caption{Results using ConvAlexNet (5 conv layers). [a] Means simple siamese. [b] Means siamese plus objectness. [c] Objectness (30 classes).}
 %[d] Means siamese with fixed reference network and objectness.}
 \begin{tabular}{cccc}
 \toprule
  Pooling & [a] & [b] & [c]\\%& [d] \\
 \midrule
  GAP & 68.0 & 72.5 & 71.2\\
  GMP & 68.4 & 70.6 & 70.7\\%& 72.0\\
 \midrule
  LENA-$0$ & 69.7 & 68.7 & 70.2 \\%& 68.3\\
  LENA-$0.5$ & 67.9 & 71.4 & 69.8\\%& 69.8 \\
  LENA-$1$ & 66.9 & 69.7 & 69.1\\%& 70.6 \\
 \bottomrule
 \end{tabular}
\end{table}

\begin{table}
 \caption{Results using MITNet (7 conv layers). [a] Means simple siamese. [b] Means siamese plus objectness.}
 \begin{tabular}{cccccc}
 \toprule
  Pooling & [a] & [b](10k) & [b](20k) & [b](30k) & [c](10k)\\
 \midrule
  GAP        & 68.0 & 71.6 & 71.0 & 71.1 & 71.1 \\
  GMP        & 71   & 71.4 & 71.2 & 71.2 & 71.6 \\
  Porzi      & 71.2 &      &      &      & 71.6 \\
 \midrule
  LENA-$0$   & 71.3 & 71.8 & 71.8 & 71.9 & 72.6 \\
  LENA-$0.5$ & 71.6 & 71.1 & 71.9 & 71.8 & 72.2 \\
  LENA-$1$   & 72.7 & 70.6 & 70.4 & 70.5 & 72.6 \\
 \bottomrule
 \end{tabular}
\end{table}

\begin{table}
 \caption{Results using ConvVGG (13 conv layers). [a] Means simple siamese. [b] Means siamese plus objectness.}
 \begin{tabular}{ccccc}
 \toprule
  Pooling & [a](10k) & [a](20k) & [a](30k) & [b] \\
 \midrule
  GAP & 71.1 & 70.8 & 70.9 & 74.1 \\
  GMP & 74.1 & 73.8 & 73.8 & 73.2\\
  Porzi & 72.4 &   &   & 74.9 \\
 \midrule
  LENA-$0$ & 73.4 & 73.7 & 73.6 & 75.6 \\
  LENA-$0.5$ & 73.4 & 74.3 & 74.2 & 74.0 \\
  LENA-$1$ & 75.7 & 74.6 & 74.5 & 74.7 \\
 \bottomrule
 \end{tabular}
\end{table}

\section{The shit}

\subsection{TODO}
\begin{itemize}
 \item Prepare annotation script. Annotate the dataset (this would also be an extra contribution).
 \item Launch Devi. Objectness and MITNet.
\end{itemize}

\subsection{Extra}
\begin{itemize}
 \item Learn deconvolution?
 \item Discuss about the fact that we are preparing objectness with 7layer convolutional alexnet and then using this objectness (also) 
with 5layer convolutional AlexNet.
\end{itemize}


\subsection{Done}
\begin{itemize}
 \item \sout{Experiments with Devi's dataset. Check with Andrea the many experiments he did and let's hope we can select a good configuration for 
us.} (Done, see below).
 \item \sout{Rank SVM experiments on new dataset (already done?).} Done
 \item \sout{Jacopo's baseline based on SIFT + bag-of-words (important: baseline for the dataset we are using).} Such baseline does not exist.
 \item \sout{Experiments with MITNet and VGG (two configs: simple siamese and simple siamese + objectness).} \sout{ Currently 
retrying AlexNet with reduced Objectness.}
 \item \sout{Reshuffle Devi's dataset. Save lmbsb'. And run SVM + features on the new split (using caffe: lr\_mult=0 (except for last fully 
conntected) + hing loss).} Done.
 \item \sout{Extract features from OUR dataset (same split as network, of course) and run SVM.} Result: 65.4\%
 \item \sout{Prepare AlexNet Objectes on Jacopo's dataset with the top 20/30.} Names: fbkvirality\_train\_obj\textbf{\_30}\_data\_lmdb
 \item \sout{Prepare Alexnet Objectness on Devi's dataset.} Done.
 \item \sout{Prepare VGG objectness on Jacopo's dataset.} Done.
 \item \sout{Launch VGG+objectness on Jacopo's dataset.} Done.
\end{itemize}
